A Framework to Learn with Interpretation

To tackle interpretability in deep learning, we present a novel framework to jointly learn a predictive model and its associated interpretation model. The interpreter provides both local and global interpretability about the predictive model in terms of human-understandable high level attribute functions, with minimal loss of accuracy. This is achieved by a dedicated architecture and well chosen regularization penalties. We seek for a small-size dictionary of high level attribute functions that take as inputs the outputs of selected hidden layers and whose outputs feed a linear classifier. We impose strong conciseness on the activation of attributes with an entropy-based criterion while enforcing fidelity to both inputs and outputs of the predictive model. A detailed pipeline to visualize the learnt features is also developed. Moreover, besides generating interpretable models by design, our approach can be specialized to provide post-hoc interpretations for a pre-trained neural network. We validate our approach against several state-of-the-art methods on multiple datasets and show its efficacy on both kinds of tasks.

==> checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \textbf{YES}
  \item Did you describe the limitations of your work?
   \textbf{YES}. Partially highlighted in conclusion, more detailed version in supplementary
  \item Did you discuss any potential negative societal impacts of your work? 
    \textbf{YES}. Please refer to the supplementary
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them? 
    \textbf{YES}
\end{enumerate}

\item The paper does NOT contain any theoretical results

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \textbf{YES}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \textbf{YES}. Please refer to supplementary for this. All details are covered
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \textbf{YES}. Mean and standard deviation for metrics on 4 runs are reported.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \textbf{YES}. Please refer to supplementary
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \textbf{YES}
  \item Did you mention the license of the assets?
   \textbf{YES}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \textbf{YES}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    All the data/code we include in supplementary is open-source.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    The data we are using does NOT contain personally identifiable information or offensive content.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \textbf{YES}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \textbf{NA}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \textbf{Ans:} The survey was completely voluntary for the participants
\end{enumerate}

\end{enumerate}
